Tensor-Based Channel Estimation and Reflection Design for RIS-Aided Millimeter-Wave MIMO Communication Systems

In this work, we consider both channel estimation and reflection design problems in point-to-point reconfigurable intelligent surface (RIS)-aided millimeter-wave (mmWave) MIMO communication systems. First, we show that by exploiting the low-rank nature of mmWave MIMO channels, the received training signals can be written as a low-rank multi-way tensor admitting a canonical polyadic CP decomposition. Utilizing such a structure, a tensor-based RIS channel estimation method (termed TenRICE) is proposed, wherein the tensor factor matrices are estimated using an alternating least squares method. Using TenRICE, the transmitter-to-RIS and the RIS-to-receiver channels are efficiently and separately estimated, up to a trivial scaling factor. After that, we formulate the beamforming and RIS reflection design as a spectral efficiency maximization problem. Due to its non-convexity, we propose a heuristic non-iterative two-step method, where the RIS reflection vector is obtained in a closed form using a Frobenius-norm maximization (FroMax) strategy. Our numerical results show that TenRICE has a superior performance, compared to benchmark methods, approaching the Cram\'er-Rao lower bound with a low training overhead. Moreover, we show that FroMax achieves a comparable performance to benchmark methods with a lower complexity.

==> acronyms.tex <==

  \begin{acronym}
  	\acro{HAD}{hybrid analog-digital}
  	\acro{FD}{fully digital}
  	\acro{SE}{spectral efficiency}
    \acro{WSR}{weighted sum rate}
  	\acro{EE}{energy efficiency }
  	\acro{DBF}{digital beamforming}
  	\acro{ABF}{analog beamforming}
  	\acro{mmWave}{millimeter-wave}
    \acro{IID}{independent and identically distributed}
  	\acro{PS}{phase-shifter}
  	
    \acro{LNA}{low-noise-amplifier}
  	\acro{ADC}{analog-to-digital converter}
  	\acro{DAC}{digital-to-analog converter}
  	\acro{PA}{power-amplifier}
  	\acro{BB}{baseband}
  	
  	
  	\acro{OMP}{orthogonal matching pursuit}
  	\acro{RHS}{right-hand-side}
  	\acro{OCI}{out-of-cell interference}

  	\acro{DBF}{digital beamforming}
  	\acro{HBF}{hybrid beamforming}

  	\acro{LoS}{Line-of-Sight}
    \acro{CS}{compressed sensing}
  	\acro{ULA}{uniform linear array}
  	\acro{BD}{block diagonalization}
  	\acro{AoD}{angle-of-departure}
  	\acro{AoA}{angle-of-arrival}
  	\acro{RF}{radio frequency}

  	\acro{3GPP}{3rd Generation Partnership Project}
  	\acro{CSI}{channel state information}
  	\acro{FDD}{frequency division duplex}
  	\acro{LTE}{long-term evolution}
  	\acro{MIMO}{Multiple-input multiple-output}
  	\acro{MRT}{maximum ratio transmission}
  	\acro{MS}{mobile station}



  	\acro{SINR}{signal-to-interference-plus-noise ratio}

  	\acro{SNR}{signal-to-noise ratio}
  	\acro{SVD}{singular value decomposition}
  	\acro{TDD}{time division duplex}
  	\acro{ZF}{zero-forcing}
  	\acro{EVD}{eigenvalue decomposition}
  	\acro{BS}{base station}
  	\acro{KKT}{karush-kuhn-tucker}
  	\acro{MSE}{mean square error}
  	\acro{MMSE}{minimum mean square error}
  	\acro{WMMSE}{weighted \ac{MMSE}}
  \end{acronym}



